Fewer Errors, but More Stereotypes? The Effect of Model Size on Gender Bias

The size of pretrained models is increasing, and so is their performance on a variety of NLP tasks. However, as their memorization capacity grows, they might pick up more social biases. In this work, we examine the connection between model size and its gender bias (specifically, occupational gender bias). We measure bias in three masked language model families (RoBERTa, DeBERTa, and T5) in two setups: directly using prompt based method, and using a downstream task (Winogender). We find on the one hand that larger models receive higher bias scores on the former task, but when evaluated on the latter, they make fewer gender errors. To examine these potentially conflicting results, we carefully investigate the behavior of the different models on Winogender. We find that while larger models outperform smaller ones, the probability that their mistakes are caused by gender bias is higher. Moreover, we find that the proportion of stereotypical errors compared to anti-stereotypical ones grows with the model size. Our findings highlight the potential risks that can arise from increasing model size.

==> 3.2_gender_errors_distribution.tex <==
Directly inferred from the above results, \textbf{as the model size increase, stereotypical errors are more prevalent than anti-stereotypical errors}
We consider the distribution of the models' gender errors (\figref{gender_error_distribution}).\roy{if you could provide a brief explanation to what this adds on top of the previous result, that would be helpful} Within all three families, larger models obtain a higher stereotypical  to anti-stereotypical error rate; in some cases, the larger models make up to 20 times more stereotypical errors than anti-stereotypical. This indicates that even though they make less gender errors, when they do make them, their mistakes are more stereotypical.\\
These results are closely related to the results on MLM experiment presented in \secref{Conflicting_results} which indicate that the large pretrained language models are more biased towards stereotypes in MLM task. According to the current results, these biases are also present in downstream task. 

